GeneSys: Enabling Continuous Learning through Neural Network Evolution in Hardware

Modern deep learning systems rely on (a) a hand-tuned neural network topology, (b) massive amounts of labeled training data, and (c) extensive training over large-scale compute resources to build a system that can perform efficient image classification or speech recognition. Unfortunately, we are still far away from implementing adaptive general purpose intelligent systems which would need to learn autonomously in unknown environments and may not have access to some or any of these three components. Reinforcement learning and evolutionary algorithm (EA) based methods circumvent this problem by continuously interacting with the environment and updating the models based on obtained rewards. However, deploying these algorithms on ubiquitous autonomous agents at the edge (robots/drones) demands extremely high energy-efficiency due to (i) tight power and energy budgets, (ii) continuous/lifelong interaction with the environment, (iii) intermittent or no connectivity to the cloud to run heavy-weight processing. To address this need, we present GENESYS, an HW-SW prototype of an EA-based learning system, that comprises a closed loop learning engine called EvE and an inference engine called ADAM. EvE can evolve the topology and weights of neural networks completely in hardware for the task at hand, without requiring hand-optimization or backpropagation training. ADAM continuously interacts with the environment and is optimized for efficiently running the irregular neural networks generated by EvE. GENESYS identifies and leverages multiple unique avenues of parallelism unique to EAs that we term 'gene'- level parallelism, and 'population'-level parallelism. We ran GENESYS with a suite of environments from OpenAI gym and observed 2-5 orders of magnitude higher energy-efficiency over state-of-the-art embedded and desktop CPU and GPU systems.

==> neat_algo.tex <==
\section{NEAT}
This is where we define the neat algorithm

==> neat_operations_table.tex <==
\begin{table}[t]
\centering
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{0pt}
\scriptsize
\begin{tabular} {|p{2cm}|p{5cm}|}
\hline
\bf Operation & \bf Description \\
\hline
Crossover & Creating a new gene by picking up attributes from parent genes based on relative fitnesses of parents  \\
\hline
Perturb mutation & Changing the attributes of the child gene by perturbing the values by small amounts \\ 
\hline
Add mutation & Addition of new gene in the child genome with default attributes.  \\
\hline
Delete mutation & Removing a node or a connection from the child genome.\\
\hline
 \end{tabular}
  \caption{\small Operations in NEAT algorithm}
  \label{table:neat_operations}
\end{table}

%
%
%% Results table:
%\begin{table*}[t]
%%\sffamily\small
%  \centering
%  % DNN name | Number of Conv/Pool/FC layers | Filter sizes
%%  \begin{tabular}{| @{~} l @{~} | r | r | r |  l | l |}
%\begin{tabular}{| @{~} p{1cm} @{~} | p{1em} | r | r |  l | l |}
%  \hline
%  % First row
%  \multicolumn{1}{@{~} c @{~}|}{\textbf{Neural Network}} &
%  \multicolumn{1}{@{~} c @{~}|}{\textbf{Num. of CONV layers}} &  
%  \multicolumn{1}{@{~} c @{~}|}{\textbf{Num. of Pool layers}} &    
%  \multicolumn{1}{@{~} c @{~}|}{\textbf{Num. of FC layers}} &    
%  \multicolumn{1}{@{~} c @{~}|}{\textbf{Filter Sizes}} &    
%  \multicolumn{1}{@{~} c @{~}|}{\textbf{Input Sizes}} \\
%  \hline
%  \hline
%  % Table entries go here
%  %%% One row of entry (example) 
%  %%%  Entry1 & Entry2 &... & Last Entry\\
%  %%%  \hline 
%  Alexnet & 6 & 1 & 1 & 11x11, 7x7, 3,3 & 224x224, 112x112, .. \\    
%  \hline    
%  \end{tabular}
%
%  \caption{Caption goes here}
%  \label{tab:motivation}
%\end{table*}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "p"
%%% End: 


==> open_ai_env_table.tex <==
\begin{table}[t]
%\centering
\center
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{0pt}
\scriptsize
\begin{tabular} {|p{1.5cm}|p{3.5cm}| p{2.5cm}|}
\hline
\bf Environment & \bf Goal & \bf Inputs \\
\hline
\textit{Acrobot}
& Balance a complex inverted pendulum constructed by linking two rigid rods 
& \squishlist
\item{\textit{Observation}: Six floating point numbers}
\item{\textit{Action}: One floating point number}
\squishend
\\
\hline
\textit{Bipedal 
}& Evolve control for locomotion of a two legged robot on a simple terrain. 
& \squishlist
\item{\textit{Observation}: Twenty four floating point numbers.}
\item{\textit{Action}: Six floating point numbers. }
\squishend  
\\ 
\hline
\textit{Cartpole\_v0} 
& The winning criteria is to balance an inverted pendulum on a moving platform for 100 consecutive time steps. & \squishlist
\item{\textit{Observation}: Four floating point numbers.}
\item{\textit{Action}: One binary value. }
\squishend
\\
\hline
\textit{MountainCar}
& The goal of this task is to control an underpowered car sitting in a valley such that it reaches the finish point on the peak of one of the mountains.
& \squishlist
\item{\textit{Observation}: Two floating point numbers.}
\item{\textit{Action}: One integer less than three, indicating the direction of motion. }
\squishend
\\
\hline
\textit{LunarLander} 
& The goal to control the landing of a module to a specific spot on the lunar surface by controlling the fire sequence of its fours thrusters. 
& \squishlist
\item{\textit{Observation}: Eight floating point numbers.}
\item{\textit{Action}: One integer less than four, indicating the thruster to fire. }
\squishend 
\\
\hline
\textit{Atari games} 
& The agent has to play Atari games by controlling button presses.
We used \textit{Airraid\_ram, Alien\_ram and Amidar\_ram} environments in our experiments 
& \squishlist
\item{\textit{Observation}: 128 bytes indicating the current state of the game RAM.}
\item{\textit{Action}: One integer value, indicating the button press. }
\squishend 
\\ 
\hline
\end{tabular}
\caption{\small Open AI environments for our experiments}
\label{table:environments}
\end{table}

%
%
%% Results table:
%\begin{table*}[t]
%%\sffamily\small
%  \centering
%  % DNN name | Number of Conv/Pool/FC layers | Filter sizes
%%  \begin{tabular}{| @{~} l @{~} | r | r | r |  l | l |}
%\begin{tabular}{| @{~} p{1cm} @{~} | p{1em} | r | r |  l | l |}
%  \hline
%  % First row
%  \multicolumn{1}{@{~} c @{~}|}{\textbf{Neural Network}} &
%  \multicolumn{1}{@{~} c @{~}|}{\textbf{Num. of CONV layers}} &  
%  \multicolumn{1}{@{~} c @{~}|}{\textbf{Num. of Pool layers}} &    
%  \multicolumn{1}{@{~} c @{~}|}{\textbf{Num. of FC layers}} &    
%  \multicolumn{1}{@{~} c @{~}|}{\textbf{Filter Sizes}} &    
%  \multicolumn{1}{@{~} c @{~}|}{\textbf{Input Sizes}} \\
%  \hline
%  \hline
%  % Table entries go here
%  %%% One row of entry (example) 
%  %%%  Entry1 & Entry2 &... & Last Entry\\
%  %%%  \hline 
%  Alexnet & 6 & 1 & 1 & 11x11, 7x7, 3,3 & 224x224, 112x112, .. \\    
%  \hline    
%  \end{tabular}
%
%  \caption{Caption goes here}
%  \label{tab:motivation}
%\end{table*}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "p"
%%% End: 

